Improving Sequence-to-Sequence Learning via Optimal Transport

Sequence-to-sequence models are commonly trained via maximum likelihood estimation (MLE). However, standard MLE training considers a word-level objective, predicting the next word given the previous ground-truth partial sentence. This procedure focuses on modeling local syntactic patterns, and may fail to capture long-range semantic structure. We present a novel solution to alleviate these issues. Our approach imposes global sequence-level guidance via new supervision based on optimal transport, enabling the overall characterization and preservation of semantic features. We further show that this method can be understood as a Wasserstein gradient flow trying to match our model to the ground truth sequence distribution. Extensive experiments are conducted to validate the utility of the proposed approach, showing consistent improvements over a wide variety of NLP tasks, including machine translation, abstractive text summarization, and image captioning.

==> alg/algorithm_sink.tex <==
% \begin{wrapfigure}[12]{R}{0.45\textwidth}
% \begin{minipage}{0.5\textwidth}
% \vspace{-12mm}
\begin{algorithm}[H]
\footnotesize
\caption{\footnotesize Sinkhorn algorithm~\citep{cuturi2013sinkhorn}}
\label{alg:sinkhorn}
\begin{algorithmic}[1]
\State {\bfseries Input:} \footnotesize{feature $\fv_1\in \sR^{n\times d}$ and $\fv_2\in \sR^{m\times d}$, $\epsilon$}
\item[]
\State $\boldsymbol{\sigma}=\mathbf{1_m}$ 
\State $\Cmat_{ij} = c(\fv_1, \fv_2)$, $\Amat_{ij} = {\rm e}^{-\frac{\Cmat_{ij}}{\epsilon}}$
\item[]
\For{$t=1,2,3\ldots$}
    % \State $\Qmat = \Amat \odot \Tmat^{(t)}$ \footnotesize{// $\odot$ is Hadamard product}
    \item[]
    \State $\boldsymbol{\delta} = \frac{1}{n\Qmat{\boldsymbol{\sigma}}}$, $\boldsymbol{\sigma} = \frac{1}{m\Qmat^\top\boldsymbol{\delta}}$
    \item[]
\EndFor

\State $\Lcal_{\text{ot}} = \langle (\Amat \odot \Cmat)\boldsymbol{\sigma}, \boldsymbol{\delta} \rangle$
\end{algorithmic}
\end{algorithm}
% \end{minipage}
%\end{wrapfigure}

==> table/DEEN.tex <==
\begin{table}[h!]
\small
\caption{Bleu score on DE-EN and EN-DE}
\label{tab:DE-EN}
\begin{center}
\begin{tabular}{lcc}
\textbf{Systems} & \textbf{NT2013} & \textbf{NT2015} \\
\hline
\textbf{Train from scratch:} & & \\ 
DE-EN: Ours NMT + OT & 28.8 &	 29.5 \\
DE-EN: NMT &	28.5 &	29.0 \\
\textbf{Train from saved model:} & & \\ 
DE-EN: Ours GNMT+OT &	29.2 &	30.1 \\
DE-EN: Pre-trained model &	29.0 &	29.9 \\
\hline
\hline
\textbf{Train from scratch:} & & \\ 
EN-DE: Ours GNMT + OT  & 24.1 &	 26.2 \\
EN-DE: GNMT  &	23.7 &	25.3 \\
\textbf{Train from saved model:} & & \\ 
EN-DE: Ours GNMT+OT & 24.6 &	 26.7 \\
EN-DE: Pre-trained model &	24.3 &	26.5 \\
\hline
\end{tabular}
\end{center}
\end{table}

==> table/SUMduc04.tex <==
\begin{table}[h!]
% \small
\caption{Rouge score on DUC2004 dataset}
\label{gigaword}
\begin{center}
\begin{tabular}{lccc}
        \hline
        \textbf{Systems} & \textbf{RG-1} & \textbf{RG-2} & \textbf{RG-L}\\
        \hline
        Seq2Seq &	28.0 &	9.4 & 24.8\\
        \textit{Seq2Seq+$\gL_{seq}$} &	29.5 &	9.8 & 25.5\\
        \textit{Seq2Seq+$\gL_{seq}$+$\gL_\text{copy}$} & \textbf{30.1} &	\textbf{10.1} & \textbf{26.0}\\
        \hline
\end{tabular}
\end{center}
\end{table}

==> table/SUMgiga.tex <==
\begin{table}[h!]
% \small
\caption{ROUGE score on different datasets}
\label{tab:gigaword}
\begin{center}
\begin{tabular}{lccc}
      \hline
        \textbf{Systems} & \textbf{RG-1} & \textbf{RG-2} & \textbf{RG-L}\\
        \hline
        Seq2Seq &	33.4 &	15.7 & 32.4\\
        \textit{Seq2Seq+$\gL_{seq}$} &	35.8 &	17.5 & 33.7\\
        \textit{Seq2Seq+$\gL_{seq}$+$\gL_\text{copy}$} &\textbf{	36.2} &\textbf{	18.1} & \textbf{34.0}\\
        \hline
      \end{tabular}
\end{center}
\end{table}

==> table/VIEN.tex <==
% \begin{table}[h!]
% \small
% \caption{Bleu score on VI-EN and EN-VI}
% \label{tab:VI-EN}
% \begin{center}
% \begin{tabular}{lcc}
% \textbf{Systems} & \textbf{newstest2012} & \textbf{newstest2013} \\
% \hline
% \textbf{Train from scratch:} & & \\
% VI-EN: Ours NMT + OT + LuongAttention (beam=10) &	21.9 &	25.0 \\
% VI-EN: NMT + LuongAttention (beam=10) &	20.7 &	23.8 \\
% \textbf{Train from saved model:} & & \\
% VI-EN: Ours NMT + OT + LuongAttention (beam=10) &	22.0 &	25.1 \\
% VI-EN: Google's pre-trained model (beam=10) &	- &	- \\
% \hline
% \hline
% \textbf{Train from scratch:} & & \\
% EN-VI: Ours NMT + OT + LuongAttention (beam=10) &	24.1 &	26.5 \\
% EN-VI: NMT + LuongAttention (beam=10) &	23.0 &	25.4 \\
% \textbf{Train from saved model:} & & \\
% EN-VI: Ours NMT + OT + LuongAttention (beam=10) &	24.5 &	26.9 \\
% EN-VI: Google's pre-trained model (beam=10) &	23.8 &	26.1 \\
% \hline
% \end{tabular}
% \end{center}
% \end{table}

\begin{table}[h!]
\small
\caption{Bleu score on VI-EN and EN-VI}
\label{tab:VI-EN}
\begin{center}
\begin{tabular}{lcc}
\textbf{Systems} & \textbf{NT2012} & \textbf{NT2013} \\
\hline
\textbf{Train from scratch:} & & \\
VI-EN: Ours NMT + OT &	21.9 &	25.0 \\
VI-EN: NMT  &	20.7 &	23.8 \\
\textbf{Train from saved model:} & & \\
VI-EN: Ours NMT + OT  &	22.0 &	25.1 \\
VI-EN: Pre-trained model &	- &	- \\
\hline
\hline
\textbf{Train from scratch:} & & \\
EN-VI: Ours NMT + OT &	24.1 &	26.5 \\
EN-VI: NMT &	23.0 &	25.4 \\
\textbf{Train from saved model:} & & \\
EN-VI: Ours NMT + OT &	24.5 &	26.9 \\
EN-VI: Pre-trained model &	23.8 &	26.1 \\
\hline
\end{tabular}
\end{center}
\end{table}

==> table/comparison.tex <==
\begin{table}%[h!]
\small
\caption{Comparison experiment}
\label{tab:toy-comparison}
\begin{center}
\begin{tabular}{lccc}
\textbf{Metric} & \textbf{Baseline} &\textbf{Case 1} & \textbf{Case 2} \\
\hline
BLEU-2 & 71.87 & 73.60 & 75.12 \\
BLEU-3 & 61.18 & 63.07 & 64.82\\
BLEU-4 & 56.59 & 58.48 & 60.27 \\
BLEU-5 & 53.73 & 55.69 & 57.50\\
\hline

\end{tabular}
\end{center}
\end{table}

==> table/softmax.tex <==

    \begin{tabular}{lcc}
        \hline
        \textbf{Systems} & \textbf{NT2012} & \textbf{NT2013} \\
        \hline
        VI-EN: GNMT  &	20.7 &	23.8 \\
        VI-EN: \textit{GNMT+OT (softmax)} &	21.8 &	24.3 \\
        VI-EN: \textit{GNMT+OT (ours)} &	21.9 &	25.5 \\
        \hline
        EN-VI: GNMT &	23.0 &	25.4 \\
        EN-VI: \textit{GNMT+OT (softmax)} &	23.5 &	26.0 \\
        EN-VI: \textit{GNMT+OT (ours)} &	24.1 &	26.5 \\
        \hline
    \end{tabular}


==> table/toy.tex <==
%
\subsection{Toy experiment}
We test our new loss using basic auto-encoder on WMT News dataset.
\begin{table}[h!]
\caption{Bleu score on WMT}
\label{AE_WMT}
\begin{center}
\begin{tabular}{lccc}
\textbf{metric} & \textbf{baseline} & \textbf{OT 1} & \textbf{OT 2}\\
\hline
Bleu-2 &	0.7187 &	0.7360 &	0.7512 \\
Bleu-3 &	0.6118 &	0.6307 &	0.6482 \\
Bleu-4 &	0.5659 &	0.5848 &	0.6027 \\
Bleu-5 &	0.5373 &	0.5569 &	0.5750 \\
\end{tabular}
\end{center}
\end{table}

\begin{table}[h!]
\caption{Bleu score on Yelp}
\label{AE_WMT}
\begin{center}
\begin{tabular}{lccc}
\textbf{metric} & \textbf{baseline} & \textbf{OT 1} & \textbf{OT 2}\\
\hline
Bleu-2 &	0.9021 &	- &	0.9093 \\
Bleu-3 &	0.7207 &	- &	0.7498 \\
Bleu-4 &	0.5055 &	- &	0.5310 \\
Bleu-5 &	0.3026 &	- &	0.3268 \\
\end{tabular}
\end{center}
\end{table}

==> table/translate.tex <==
\begin{table}[t!]
\footnotesize
    % \caption{Global caption}
    \begin{minipage}{.5\linewidth}
      \caption{BLEU scores on VI-EN and EN-VI.}
      \vspace{0.05in}
      \label{tab:VI-EN}
      \centering
        \begin{tabular}{lcc}
        \hline
        \textbf{Systems} & \textbf{NT2012} & \textbf{NT2013} \\
        \hline
        \textbf{Train from scratch:} & & \\
        VI-EN: NMT  &	20.7 &	23.8 \\
        VI-EN: \textit{NMT+OT (Ours)} &	21.9 &	25.5 \\
        \textbf{Fine-tune:} & & \\
        VI-EN: Pre-trained model &	- &	- \\
        VI-EN: \textit{NMT+OT (Ours)} &	\textbf{22.0} &\textbf{	25.6} \\
        \hline
        \textbf{Train from scratch:} & & \\
        EN-VI: NMT &	23.0 &	25.4 \\
        EN-VI: \textit{NMT+OT (Ours)} &	24.1 &	26.5 \\
        \textbf{Fine-tune:} & & \\
        EN-VI: Pre-trained model &	23.8 &	26.1 \\
        EN-VI: \textit{NMT+OT (Ours)} &	\textbf{24.5} &	\textbf{26.9} \\
        \hline
        \end{tabular}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
      \centering
        \caption{BLEU scores on DE-EN and EN-DE.}
        \vspace{0.05in}
        \label{tab:DE-EN}
        \begin{tabular}{lcc}
        \hline
        \textbf{Systems} & \textbf{NT2013} & \textbf{NT2015} \\
        \hline
        \textbf{Train from scratch:} & & \\ 
        DE-EN: GNMT &	28.5 &	29.0 \\
        DE-EN: \textit{GNMT+OT (Ours)} & 28.8 &	 29.5 \\
        \textbf{Fine-tune:} & & \\ 
        DE-EN: Pre-trained model &	29.0 &	29.9 \\
        DE-EN: \textit{GNMT+OT (Ours)}&	\textbf{29.2} &	\textbf{30.1} \\
        \hline
        \textbf{Train from scratch:} & & \\ 
        EN-DE: GNMT  &	23.7 &	25.3 \\
        EN-DE: \textit{GNMT+OT (Ours)}  & 24.1 &	 26.2 \\
        \textbf{Fine-tune:} & & \\ 
        EN-DE: Pre-trained model &	24.3 &	26.5 \\
        EN-DE: \textit{GNMT+OT (Ours)}& \textbf{24.6} &	 \textbf{26.7} \\
        % EN-DE: Ours GNMT+OT & 26.1 &	 28.0 \\
        % EN-DE: Pre-trained model &	25.6 &	27.6 \\
        \hline
        \end{tabular}
    \end{minipage} 
\end{table}
